How to Train your DNN: The Network Operator Edition

Deep Neural Nets have hit quite a crest, But physical networks are where they must rest, And here we put them all to the test, To see which network optimization is best.

==> analytical_model.tex <==
\section{Appendix: Analytical Model}
\label{sec:analytical_framework}

We develop a simple analytical model. This model does not account for performance and transfer time variations between workers and between parameter servers (\ie it assumes that all workers execute at the same rate and transfer data at the same rate, and the same for parameter servers). In modeling DNN performance we need to account for pipelining. We observe that training algorithms allow distribution to be interleaved with forward pass, and backpropagation to be interleaved with aggregation. Backpropagation requires use of results computed as a part of forward pass and hence these steps cannot be interleaved. Based on this observation, we split iteration times into two groups -- distribution and forward pass time $D$, and backpropagation and aggregation time $A$. Assuming that parameter servers send layers in order, distribution and forward pass time $D$ can be approximated as $D = t_d(l_0) + max(c_f(m), \sum_{i=1\ldots n}t_d(l_i))$ where $t_d(l_i)$ is the time taken to transfer layer $l_i$ from the parameter server to workers (we assume all workers are symmetric in this model), and $c_f(m)$ is the overall forward pass time for the model as a whole. The $max$ term accounts for pipelining by capturing the fact that overall time depends on whether communication ($\sum t_d(l_i)$) or computation $(c_f(m)$) is the bottleneck. Simplifying this further we can approximate $D\approx max(c_f(m), t_d(m))$ where $t_d(m)$ represents the distribution time for the model. Similarly, backpropagation and aggregation time, $A$, can be expressed as $A \approx max(c_b(m), t_a(m))$, where $c_b(m)$ is the backpropagation time for model $m$ and $t_a(m)$ is time taken for transferring updates from workers to the parameter server. Thus, this model approximates the training time by $A+D \approx max(c_f(m), t_d(m)) + max(c_b(m), t_a(m))$.

To demonstrate the utility of our model, we begin by comparing the effect of improving communication time for distribution and aggregation. We make a series of assumptions here that we will later relax in our simulations. First, assume that computation time $c_f$ and $c_b$ are invariant with improved communication. Secondly, assume a simple topology where machines are connected by a full-bisection network, and a set of homogeneous nodes. Consider a run with $w$ workers and one parameter server. Given this setting, it is simple to observe that distribution and aggregation times are dominated by the time it takes to transfer data from the worker to the parameter server. More specifically, under these assumptions where point-to-point connections are used to transfer data, a total of $w\cdot m$ bytes of data must be transferred across the link (we assume $m$ is model size), and takes $\frac{w\cdot m}{b}$ seconds, where $b$ is the bandwidth available on the link connecting the parameter server to the network fabric. When using multiple parameter servers, our analytical model assumes the model is evenly split across the parameter servers, and hence data transfer in each step takes $\frac{w\cdot m}{p\cdot b}$ seconds with $p$ parameter servers.

Now consider two network modifications to improve performance: the first uses multicast to reduce distribution time, and the second uses in-network aggregation to improve aggregation time. In either case, transfer time for the affected step reduces from $\frac{w \cdot m}{b}$ to $\frac{m}{b}$ when these techniques are applied. Subsequently, we consider the original question: how do we assess the relative importance of the distribution phase and the aggregation phase? Ultimately, we plugged in some empirical data from Resnet-200. 
\begin{itemize}
    \item Model size $m$ is 200MB. 
    \item Forward pass time $c_f$ is 169.62ms, while backpropagation time $c_b$ is 383.80ms. 
    \item Runs in an environment with $25$Gbps links.
\end{itemize}
\begin{figure*}[th]
\minipage{0.31\textwidth}
    \includegraphics[width=\textwidth]{plots/cdf/res101.pdf}
    \caption{CDF of time taken for each training iteration when training Resnet-101.}
    \vspace{-.1in}
    \label{fig:res101-cdf}
\endminipage\hfill
\minipage{0.31\textwidth}
    \includegraphics[width=\linewidth]{plots/inception_weight_distribution.pdf}
    \caption{Layers in the Inception-v3 model are small until the last layer}
    \vspace{-.1in}
    \label{fig:inception-weight-distribution}
\endminipage\hfill
\minipage{0.31\textwidth}
    \includegraphics[width=\linewidth]{plots/vgg_weight_distribution.pdf}
    \caption{Layers in the VGG-16 model are also small until the last layer}
    \vspace{-.1in}
    \label{fig:vgg-weight-distribution}
\endminipage\hfill
\end{figure*}

\begin{figure*}[th]
\minipage{0.31\textwidth}
    \includegraphics[width=\linewidth]{plots/resnet-200_hockey.pdf}
    \caption{Results of simple analytic model from Resnet-200. Forward pass and backpropagation data profiled on Maxwell Titan X GPU}
    \vspace{-.1in}
    \label{fig:resnet-200-hockey}
\endminipage\hfill
\minipage{0.31\textwidth}
    \includegraphics[width=\linewidth]{plots/vgg16_hockey.pdf}
    \caption{Results of the simple analytic model from VGG-16. Forward pass and backprop data profiled on Maxwell Titan X GPU}
    \vspace{-.1in}
    \label{fig:VGG-16-hockey}
\endminipage\hfill
\minipage{0.31\textwidth}
    \includegraphics[width=\textwidth]{plots/cdf/iv3.pdf}
    \caption{CDF of time taken for each training iteration when training Inception-v3.}
    \vspace{-.1in}
    \label{fig:iv3-cdf}
\endminipage
\end{figure*}

\begin{table}[t]
\centering
\footnotesize
% \resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lrrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{DNN Name}} & \multicolumn{1}{c}{\textbf{GPU Model}} & \multicolumn{1}{c}{\textbf{Forward Pass}} & \multicolumn{1}{c}{\textbf{Backprop}}\\ \midrule
Resnet-200            & Maxwell Titan X          & 169.62 ms & 383.8  ms  \\
Resnet-200            & Pascal Titan X          & 314.77 ms & 519.72 ms\\
VGG-16            & Maxwell Titan X          & 172.61 ms & 415.87 ms  \\
VGG-16            & Pascal Titan X          & 98.15 ms & 260.38  ms \\
Resnet-101       & Maxwell Titan X        & 108.96 ms & 189.93 ms \\
Resnet-101      & Pascal Titan X          & 161.55 ms & 257.57 ms \\
Inception-v1       & Maxwell Titan X        & 91.31 ms & 140.81 ms \\
Inception-v1      & Pascal Titan X          & 57.46 ms & 85.90 ms \\
\end{tabular}%}
\caption{Forward Pass vs. Backpropagation Benchmarks \cite{cnnbenchmark}}
\label{fwd_pass_benchmarks}
\vspace{-0.2in}
\end{table}


The results for this are shown in Figure \ref{fig:resnet-200-hockey}. Note that this graph has a characteristic ``hockey stick" shape, where for small numbers of workers improving the network does not help at all, but for larger number of workers the impact increases linearly with the number of workers. Despite all the simplifications in our model, this shape holds even for more realistic simulations (to be described later).%\fixme{is this ok??}

Observe that backpropagation time is more than $2\times$ larger than forward pass time. Primarily based on this observation, when we compare the overall benefits of using multicast versus in-network aggregation, our model predicts that multicast should help in any scenario where 3 or more workers are used for training, while in-network aggregation only shows benefits with 6 or more workers.  This is in contrast to the VGG-16 model (shown in Figure \ref{fig:VGG-16-hockey}). Despite exhibiting the same ratio between backpropagation time and forward pass time, the VGG-16 model (shown in Figure \ref{fig:VGG-16-hockey}) is $4\times$ the size of
Resnet-200 which adds to the network transmission delay. In this case, multicast is expected to help even in a unrealistic distributed cluster of one worker, while network overhead in the aggregation phase would appear when using two worker machines. We also applied this same line of reasoning to a variety of other models and find that our observations generalize. Table \ref{fwd_pass_benchmarks} shows benchmarks across various DNN and GPU pairings, and shows that backpropagation is typically in the range of 1.5x-2x longer in duration than the forward pass.

However, this simple model does not account for a variety of factors that impact performance including:
\begin{compactenum}
    \item \textbf{Network Variability:} The previous model assumes all workers receive model parameters at the same time. In reality this is not true; for example, we have observed that two workers will receive the same layer as much as a whole second apart in reasonably sized clusters of 8 workers running the Inception-v3 model. While this has no effect on our modeling of the distribution phase, the network overhead of the aggregation phase is most significant when the workers are sending their updates to the parameter server at the exact same time.
    \item \textbf{Computation Variability:} The previous model assumes that computation times are constant across different worker machines. Empirically this is not true as demonstrated by the cumulative distribution functions (CDFs) in Figure~\ref{fig:iv3-cdf} and Figure~\ref{fig:res101-cdf}. Figure~\ref{fig:iv3-cdf} shows that iteration times exhibit a long tail when training DNNs like Inception-v3, while Figure~\ref{fig:res101-cdf} shows that other models such as Resnet-101 exhibit highly variable iteration times.
    \item \textbf{Variability in Layer Sizes:} Individual layers in a model show wide variance in size. For example in VGG-16 the largest layer is 53MB, while the smallest layer is only 1KB. As a result of this difference in sizes, pipelining is often imperfect.
    \item \textbf{Multiple Parameter Servers:} It is common to deploy multiple parameter servers to reduce contention on the parameter server link. This model fails to account for the effects of using multiple parameter servers and how the parameters are sharded among the parameter servers.
\end{compactenum}

While the analytical formulation provides some intuition on the relationship between the compute steps and the network step, it does not fully capture the context around the communication, making it challenging to reason about its effect on the end-to-end iteration training time. A more sophisticated model is needed, which we describe in the next section. 

==> tables/inception-model-complexity.tex <==
\begin{tabular}{|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{Inception-v3 Model Complexity} \\
    \hline
    Layer & \# of Weights & Bytes of Weights & \# of FLOPs \\
    \hline
    conv0 & 288 & 1152 & 38363328 \\
    conv1 & 288 & 1152 & 398297088 \\
    conv2 & 576 & 2304 & 796594176 \\
    pool1 & 0 & 0 & 3069504 \\
    conv3 & 80 & 320 & 54568960 \\
    conv4 & 1728 & 6912 & 1393735680 \\
    pool2 & 0 & 0 & 2116800 \\
    mixed & 3536 & 14144 & 628924800 \\
    mixed\_1 & 3568 & 14272 & 683020800 \\
    mixed\_2 & 3568 & 14272 & 702542400 \\
    mixed\_3 & 5248 & 20992 & 804623904 \\
    mixed\_4 & 6912 & 27648 & 752121344 \\
    mixed\_5 & 7872 & 31488 & 979400192 \\
    mixed\_6 & 7872 & 31488 & 979400192 \\
    mixed\_7 & 8832 & 35328 & 1239823872 \\
    aux\_logits & 788096 & 3152384 & 7451136 \\
    mixed\_8 & 7680 & 30720 & 582451200 \\
    mixed\_9 & 9408 & 37632 & 646348800 \\
    mixed\_10 & 9408 & 37632 & 779354112 \\
    logits & 1640038.4 & 6560153.6 & 4369339 \\
    \hline
\end{tabular}

==> tables/vgg16-model-complexity.tex <==
\begin{tabular}{|c|c|c|c|}
    \hline
    \multicolumn{4}{|c|}{VGG-16 Model Complexity} \\
    \hline
    Layer & \# of Weights & Bytes of Weights & \# of FLOPs \\
    \hline
    conv0 & 576 & 2304 & 308969856 \\
    conv1 & 576 & 2304 & 6591356928 \\
    pool1 & 0 & 0 & 11366912\\
    conv2 & 1152 & 4608 & 3273670656 \\
    conv3 & 1152 & 4608 & 6547341312 \\
    pool2 & 0 & 0 & 5607424 \\
    conv4 & 2304 & 9216 & 3229876224 \\
    conv5 & 2304 & 9216 & 6459752448 \\
    conv6 & 2304 & 9216 & 6459752448 \\
    pool3 & 0 & 0 & 2803712 \\
    conv7 & 4608 & 18432 & 3229876224 \\
    conv8 & 4608 & 18432 & 6459752448 \\
    conv9 & 4608 & 18432 & 6459752448 \\
    pool4 & 0 & 0 & 1327104 \\
    conv10 & 4608 & 18432 & 1528823808 \\
    conv11 & 4608 & 18432 & 1528823808 \\
    conv12 & 4608 & 18432 & 1528823808 \\
    pool5 & 0 & 0 & 331776 \\
    fc1 & 169869312 & 679477248 & 339738624 \\
    dropout1 & 0 & 0 & 8192 \\
    fc2 & 13421772.8 & 53687091.2 & 33554432 \\
    dropout2 & 0 & 0 & 8192 \\
    logits & 3280076.8 & 13120307.2 & 8200192 \\
    \hline
\end{tabular}
